How Transferable are Attribute Controllers on Pretrained Multilingual Translation Models?

Customizing machine translation models to comply with desired attributes (e.g., formality or grammatical gender) is a well-studied topic. However, most current approaches rely on (semi-)supervised data with attribute annotations. This data scarcity bottlenecks democratizing such customization possibilities to a wider range of languages, particularly lower-resource ones. This gap is out of sync with recent progress in pretrained massively multilingual translation models. In response, we transfer the attribute controlling capabilities to languages without attribute-annotated data with an NLLB-200 model as a foundation. Inspired by techniques from controllable generation, we employ a gradient-based inference-time controller to steer the pretrained model. The controller transfers well to zero-shot conditions, as it operates on pretrained multilingual representations and is attribute -- rather than language-specific. With a comprehensive comparison to finetuning-based control, we demonstrate that, despite finetuning's clear dominance in supervised settings, the gap to inference-time control closes when moving to zero-shot conditions, especially with new and distant target languages. The latter also shows stronger domain robustness. We further show that our inference-time control complements finetuning. A human evaluation on a real low-resource language, Bengali, confirms our findings. Our code is https://github.com/dannigt/attribute-controller-transfer

==> data_overview.tex <==
\begin{table}[t]
\small
\centering
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{tabular}{lllr}
\toprule
\multicolumn{2}{l}{\textbf{Task}} & 
\textbf{Directions} & 
\textbf{\# Sent.} \\
\midrule
\multicolumn{3}{l}{\textbf{Formality control} (formal/informal)} \\
&
train & 
en$\rightarrow$\{de, es, fr, hi, it\} &
400
\\
& test (supervised)
& en$\rightarrow$\{de, es, fr, hi, it\} 
& 600
\\
& test (new tgt)
& en$\rightarrow$\{pt, ru, ko\}
& 600
\\
%\multirow{2}{*}{
&\multirow{2}{*}{\shortstack[l]{test (new src)}}
%}
&\multirow{2}{*}{\shortstack[l]{${s}\rightarrow{t}$ for $s,t\in$ \{de, 
\\
es, fr, hi, it\}, $s \ne t$}}
&\multirow{2}{*}{\shortstack[r]{366-572}}
\\\\
\multicolumn{4}{l}{\textbf{Grammatical gender control} (feminine/masculine)} \\
& train 
& en$\rightarrow$es
& 194
\\
&
test (supervised)
& 
en$\rightarrow$es
& 552-556 %\verb|~|
\\
&
test (new tgt)
& en$\rightarrow$\{it, fr\}
& 515-546
\\
&
test (new src \& tgt)
&\{es, fr\}$\rightarrow$it, \{es, it\}$\rightarrow$fr 
& 271-365
\\
\bottomrule
\end{tabular}
\caption{\label{tab:data_overview} 
Data overview.
Abbreviations: English (en), German (de), Spanish (es), French (fr), Hindi (hi), Italian (it), Korean (ko), Portuguese (pt), Russian (ru),  source (src), target (tgt).
Last column shows data amount for \textit{each attribute}.
}
\end{table}

==> tables/formality_control_supervised.tex <==

\begin{table*}[h]
\small
\centering
\setlength\tabcolsep{2.5pt} % default value: 6pt
\begin{tabular}{lccc|ccc|ccc|ccc|ccc|cc}
%\toprule& 
&
\multicolumn{3}{c}{\textbf{en$\rightarrow$de}} & 
\multicolumn{3}{c}{\textbf{en$\rightarrow$es}} & 
\multicolumn{3}{c}{\textbf{en$\rightarrow$fr}} & 
\multicolumn{3}{c}{\textbf{en$\rightarrow$hi}} & 
\multicolumn{3}{c}{\textbf{en$\rightarrow$it}} & 
\multicolumn{2}{c}{\textbf{Average}} \\
\textbf{ID} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} &
\textbf{F} & 
\textbf{I} \\ 
\hline
%\multicolumn{5}{l}{From ground-truth transcripts (\textbf{MT alone})} \\
NLLB-200 
& 45.6
& 54.4
& $-$
& 29.7
& 70.3
& $-$
& 76.8
& 23.2
& $-$
& 96.7
& 3.3
& $-$
& 3.2
& 96.8
& $-$\\
BLEU/COMET
& \multicolumn{2}{c}{35.7{\color{gray!80}\scriptsize$\pm$1.0}}
& 0.821
& \multicolumn{2}{c}{40.0{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.839
& \multicolumn{2}{c}{36.0{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.808
& \multicolumn{2}{c}{24.0{\color{gray!80}\scriptsize$\pm$0.9}}
& 0.755
& \multicolumn{2}{c}{41.3{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.849
\\
+ class. guidance
& 95.0
& 89.6
& 92.3
& 72.9
& 92.4
& 82.7
& 99.8
& 77.2
& 88.5
& 99.3
& 30.7
& 65.0
& 18.7 
& 99.5
& 59.1
\\
BLEU/COMET
& \multicolumn{2}{c}{38.4{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.816
& \multicolumn{2}{c}{41.2{\color{gray!80}\scriptsize$\pm$1.2}}
& 0.844
& \multicolumn{2}{c}{38.8{\color{gray!80}\scriptsize$\pm$1.2}}
& 0.809
& \multicolumn{2}{c}{24.3{\color{gray!80}\scriptsize$\pm$0.9}}
& 0.750
& \multicolumn{2}{c}{40.6{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.841
%\bottomrule
\end{tabular}
\caption{\label{tab:formality_supervised} Supervised classifier guidance results.}
\end{table*}

==> tables/formality_control_zs_source.tex <==

\begin{table*}[h]
\small
\centering
\setlength\tabcolsep{3pt} % default value: 6pt
\begin{tabular}{lccc|ccc|ccc|ccc|ccc|cc}
%\toprule& 
&
\multicolumn{3}{c}{\textbf{X$\rightarrow$de}} & 
\multicolumn{3}{c}{\textbf{X$\rightarrow$es}} & 
\multicolumn{3}{c}{\textbf{X$\rightarrow$fr}} & 
\multicolumn{3}{c}{\textbf{X$\rightarrow$hi}} & 
\multicolumn{3}{c}{\textbf{X$\rightarrow$it}} &
\multicolumn{2}{c}{\textbf{Average}}\\
\textbf{ID} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} & 
\textbf{Avg} & 
\textbf{F} & 
\textbf{I} &  
\textbf{Avg} &
\textbf{F} & 
\textbf{I} \\ 
\hline
%\multicolumn{5}{l}{From ground-truth transcripts (\textbf{MT alone})} \\
\textbf{Source\colorbox{gray!30}{formal}} \\
NLLB-200 
&\cellcolor[HTML]{d3d1d1}77.8
& 22.2
& $-$  
&\cellcolor[HTML]{d3d1d1}57.8
& 42.2
& $-$
&\cellcolor[HTML]{d3d1d1}97.0
& 3.0
& $-$
&\cellcolor[HTML]{d3d1d1}98.2
& 1.8
& $-$
&\cellcolor[HTML]{d3d1d1}23.0
& 77.0
& $-$\\
BLEU/COMET
& \multicolumn{2}{c}{23.9{\color{gray!80}\scriptsize$\pm$0.5}}
& 0.790
& \multicolumn{2}{c}{29.8{\color{gray!80}\scriptsize$\pm$0.5}}
& 0.827
& \multicolumn{2}{c}{29.5{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.791
& \multicolumn{2}{c}{20.2{\color{gray!80}\scriptsize$\pm$0.4}}
& 0.732
& \multicolumn{2}{c}{27.6{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.835
\\
+ class. guidance
&\cellcolor[HTML]{d3d1d1}98.6
& 71.5
& 85.0
&\cellcolor[HTML]{d3d1d1}86.7
& 73.3
& 80.0
&\cellcolor[HTML]{d3d1d1}99.8
& 40.4
& 70.1
&\cellcolor[HTML]{d3d1d1}99.2
& 9.8
& 54.5
&\cellcolor[HTML]{d3d1d1}45.8
& 88.1
& 67.0\\
BLEU/COMET
& \multicolumn{2}{c}{25.9{\color{gray!80}\scriptsize$\pm$0.5}}
& 0.787
& \multicolumn{2}{c}{30.5{\color{gray!80}\scriptsize$\pm$0.8}}
& 0.823 
& \multicolumn{2}{c}{30.6{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.789
& \multicolumn{2}{c}{20.3{\color{gray!80}\scriptsize$\pm$0.4}}
& 0.730
& \multicolumn{2}{c}{28.1{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.829
\\
\hline
\textbf{Source\colorbox{blue!15}{informal}} \\
NLLB-200 
& 48.5
& \cellcolor{blue!15}51.5
& $-$
& 20.3
& \cellcolor{blue!15}79.7
& $-$
& 87.7
& \cellcolor{blue!15}12.3
& $-$
& 98.4
& \cellcolor{blue!15}1.6
& $-$
& 1.5
& \cellcolor{blue!15}98.5
& $-$\\
BLEU/COMET
& \multicolumn{2}{c}{24.7{\color{gray!80}\scriptsize$\pm$0.5}}
& 0.793 
& \multicolumn{2}{c}{29.9{\color{gray!80}\scriptsize$\pm$0.5}}
& 0.827
& \multicolumn{2}{c}{30.3{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.796
& \multicolumn{2}{c}{20.8{\color{gray!80}\scriptsize$\pm$0.4}}
& 0.736
& \multicolumn{2}{c}{28.0{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.836
\\
+ class. guidance
& 94.0
& \cellcolor{blue!15}87.7
& 90.8
& 67.5
& \cellcolor{blue!15}93.7
& 80.6
& 99.9
& \cellcolor{blue!15}59.5
& 79.7
& 99.2
& \cellcolor{blue!15}12.3
& 55.7
& 17.1
& \cellcolor{blue!15}99.4
& 58.2
\\
BLEU/COMET
& \multicolumn{2}{c}{27.0{\color{gray!80}\scriptsize$\pm$0.5}}
& 0.790
& \multicolumn{2}{c}{31.1{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.823
& \multicolumn{2}{c}{32.5{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.796
& \multicolumn{2}{c}{20.8{\color{gray!80}\scriptsize$\pm$0.4}}
& 0.734
& \multicolumn{2}{c}{28.0{\color{gray!80}\scriptsize$\pm$0.6}}
& 0.829
\\
\end{tabular}
\caption{\label{tab:formality_src_zs} Source side zero-shot formality control results.}
\end{table*}


==> tables/formality_control_zs_target.tex <==
\begin{table}[ht!]
\small
\centering
\setlength\tabcolsep{3.5pt} % default value: 6pt
\begin{tabular}{lccc|ccc}
%\toprule& 
&
\multicolumn{3}{c}{\textbf{en$\rightarrow$pt}} & 
\multicolumn{3}{c}{\textbf{en$\rightarrow$ru}} \\
\textbf{ID} & 
\textbf{I} & 
\textbf{F} & 
\textbf{Avg} & 
\textbf{I} & 
\textbf{F} &
\textbf{Avg} \\ 
\hline
%\multicolumn{5}{l}{From ground-truth transcripts (\textbf{MT alone})} \\
NLLB-200 
& 47.7
& 52.3
& $-$
& 55.0
& 45.0
& $-$ \\
BLEU/COMET
& \multicolumn{2}{c}
{41.7{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.851 
& \multicolumn{2}{c}
{30.3{\color{gray!80}\scriptsize$\pm$1.0}}
& 0.837 \\
+ CG (es)
& 85.4
& 83.6
& \textbf{84.5}
& 86.8
& 73.9
& 80.4 \\
BLEU/COMET
& \multicolumn{2}{c}
{43.8{\color{gray!80}\scriptsize$\pm$1.0}}
& 0.850
& \multicolumn{2}{c}
{32.4{\color{gray!80}\scriptsize$\pm$1.0}}
& 0.832
\\
+ CG (fr)
& 86.2
& 67.7
& 77.0
& 93.7
& 79.3
& \textbf{86.5} \\
BLEU/COMET
& \multicolumn{2}{c}
{43.2{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.848
& \multicolumn{2}{c}
{32.6{\color{gray!80}\scriptsize$\pm$1.0}}
& 0.831 
\\
+ CG (de)
& 75.6
& 74.2
& 74.9
& 87.3
& 77.7
& 82.5 \\
BLEU/COMET
& \multicolumn{2}{c}
{43.0{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.849
& \multicolumn{2}{c}
{32.2{\color{gray!80}\scriptsize$\pm$1.0}}
& 0.831
\\
+ CG (multi5)
& 84.8
& 80.0
& 82.4
& 87.3
& 78.2
& 82.8 \\
BLEU/COMET
& \multicolumn{2}{c}
{43.7{\color{gray!80}\scriptsize$\pm$1.1}}
& 0.849
& \multicolumn{2}{c}
{32.2{\color{gray!80}\scriptsize$\pm$1.0}}
& 0.832
\\
%\bottomrule
\end{tabular}
\caption{\label{tab:formality_tgt_zs} Target side zero-shot formality control  results.}
\end{table}
